FELM: Benchmarking Factuality Evaluation of Large Language Models

Assessing factuality of text generated by large language models (LLMs) is an emerging yet crucial research area, aimed at alerting users to potential errors and guiding the development of more reliable LLMs. Nonetheless, the evaluators assessing factuality necessitate suitable evaluation themselves to gauge progress and foster advancements. This direction remains under-explored, resulting in substantial impediments to the progress of factuality evaluators. To mitigate this issue, we introduce a benchmark for Factuality Evaluation of large Language Models, referred to as felm. In this benchmark, we collect responses generated from LLMs and annotate factuality labels in a fine-grained manner. Contrary to previous studies that primarily concentrate on the factuality of world knowledge (e.g.~information from Wikipedia), felm focuses on factuality across diverse domains, spanning from world knowledge to math and reasoning. Our annotation is based on text segments, which can help pinpoint specific factual errors. The factuality annotations are further supplemented by predefined error types and reference links that either support or contradict the statement. In our experiments, we investigate the performance of several LLM-based factuality evaluators on felm, including both vanilla LLMs and those augmented with retrieval mechanisms and chain-of-thought processes. Our findings reveal that while retrieval aids factuality evaluation, current LLMs are far from satisfactory to faithfully detect factual errors.

==> tables/questions.tex <==
% \begin{table*}[t]
% 	\small
% 	\centering
% 	% \begin{tabular}{p \textwidth}
%  \begin{tabular}{p {0.95\textwidth}}
% 		\toprule
%          \colorbox{tOrange}{\fontfamily{put}\selectfont \textbf{World Knowledge}}\\
%            \specialrule{0em}{1pt}{1pt}
%             {\fontfamily{put}\selectfont \faCaretRight  \quad Which country or city has the maximum number of nuclear power plants? } \\
%              \specialrule{0em}{1pt}{1pt}
%              {\fontfamily{put}\selectfont \faCaretRight \quad Why was it illegal for black people to attend the university of Alabama in 1984? } \\
            
%  \specialrule{0em}{1pt}{1pt}
% % \midrule
   
%             \colorbox{tGreen}{\fontfamily{put}\selectfont \textbf{Science/Tech}}\\
%              \specialrule{0em}{1pt}{1pt}
%             {\fontfamily{put}\selectfont 
%             \faCaretRight  \quad What is the chemical composition of the atmosphere on Jupiter's moon Europa?}\\
%             \specialrule{0em}{1pt}{1pt}
%             {\fontfamily{put}\selectfont 
%             \faCaretRight  \quad What is PPO algorithm?}\\
%            \specialrule{0em}{1pt}{1pt}
%               \colorbox{tPink}{\fontfamily{put}\selectfont \textbf{Recommendation}}\\
%               \specialrule{0em}{1pt}{1pt}
%             {\fontfamily{put}\selectfont 
%             \faCaretRight  \quad Can you recommend me some sci-fi movies?}\\
%              \specialrule{0em}{1pt}{1pt}
%              {\fontfamily{put}\selectfont 
%             \faCaretRight  \quad Can you suggest some good vegan restaurants in my area? I am in downtown Los Angeles.}\\

%              \specialrule{0em}{1pt}{1pt}
%               \colorbox{tBlue}{\fontfamily{put}\selectfont \textbf{Writing}}\\
%               \specialrule{0em}{1pt}{1pt}
%             {\fontfamily{put}\selectfont \faCaretRight  \quad Please write a biography of Gary Smith, a professor of economics at Pomona College.}\\
%              \specialrule{0em}{1pt}{1pt}
%              {\fontfamily{put}\selectfont \faCaretRight  \quad Review a popular computer software or application, and evaluate its functionality, user interface, and overall value for users.}\\
%          \specialrule{0em}{1pt}{1pt}
%               \colorbox{tPurple}{\fontfamily{put}\selectfont \textbf{Math}}\\
%                \specialrule{0em}{1pt}{1pt}
%             {\fontfamily{put}\selectfont \faCaretRight  \quad Show me the answer for the following math question: 143287*534156=?}\\
%              \specialrule{0em}{1pt}{1pt}
%              {\fontfamily{put}\selectfont \faCaretRight  \quad Tell me the answer to 2+4*3-7=? }\\
%               \specialrule{0em}{1pt}{1pt}
%                \colorbox{tGold}{\fontfamily{put}\selectfont \textbf{Reasoning}}\\
%                \specialrule{0em}{1pt}{1pt}
%             {\fontfamily{put}\selectfont \faCaretRight  \quad What is the fifth word of this sentence?}\\
%              \specialrule{0em}{1pt}{1pt}
%              {\fontfamily{put}\selectfont \faCaretRight  \quad Can you put seven blue balls and two red balls into a tube that holds seven balls?} 
%             % \rowcolor{tGreen}{\fontfamily{ppl}\selectfont He currently holds a position as an associate professor at the Language Technologies Institute in Carnegie Mellon University's School of Computer Science.}\\
%             %  \\
%             % \rowcolor{tPink}{\fontfamily{ppl}\selectfont Neubig is known for his contributions to machine translation, specifically in the area of low-resource machine translation, which involves developing translation systems for languages with limited amounts of available data.}\\
%             % \\
%             % \rowcolor{tPink}{\fontfamily{ppl}\selectfont He has also contributed to the development of tools and resources for NLP researchers, including the widely-used programming language for NLP research, PyTorch.}\\
%             % \\
%             % \rowcolor{tGreen}{\fontfamily{ppl}\selectfont Neubig has published numerous research papers and has spoken at several conferences on NLP and machine learning.}
%             % \specialrule{0em}{1pt}{1pt}
%             % \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{\#Knowledge\#:} The nine mile byway starts south of Morehead, Kentucky and can be accessed by U.S. Highway 60. Morehead is a home rule-class city located along US 60 (the historic Midland Trail) and Interstate 64 in Rowan County, Kentucky, in the United States.} \\
%             % \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{\#Question\#:} What U.S Highway gives access to Zilpo Road, and is also known as Midland Trail?} \\
%             % \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{\#Right Answer\#:} U.S. Highway 60 } \\
%             % \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{\#Hallucinated Answer\#:} U.S. Highway 70} \\
%             % {\fontfamily{ppl}\selectfont or} \\
%             % \rowcolor{tPink}{\fontfamily{ppl}\selectfont You are trying to answer a question but you misunderstand the question context and intention.} \\
%             % \specialrule{0em}{1pt}{1pt}
%             % \rowcolor{tGreen}{\fontfamily{ppl}\selectfont <Demonstrations>} \\
%             % {\fontfamily{ppl}\selectfont or} \\
%             % \rowcolor{tPink}{\fontfamily{ppl}\selectfont You are trying to answer a question but the answer is too general or too specific to answer the question at an appropriate level of specificity.} \\
%             % \specialrule{0em}{1pt}{1pt}
%             % \rowcolor{tGreen}{\fontfamily{ppl}\selectfont <Demonstrations>} \\
%             % {\fontfamily{ppl}\selectfont or} \\
%             % \rowcolor{tPink}{\fontfamily{ppl}\selectfont You are trying to answer a question but the answer cannot be inferred from the knowledge. You can incorrectly reason with the knowledge to arrive at a hallucinated answer.} \\
%             % \specialrule{0em}{1pt}{1pt}
%             % \rowcolor{tGreen}{\fontfamily{ppl}\selectfont <Demonstrations>} \\
%             % \\
%             % {\fontfamily{ppl}\selectfont You should try your best to make the answer become hallucinated. \#Hallucinated Answer\# can only have about 5 more words than \#Right Answer\#. } \\
%             % \\
%             % {\fontfamily{ppl}\selectfont \textbf{\#Knowledge\#:} <Here is the related knowledge>} \\
%             % {\fontfamily{ppl}\selectfont \textbf{\#Question\#:} <Here is the test question>} \\
%             % {\fontfamily{ppl}\selectfont \textbf{\#Right Answer\#:} <Here is the right answer to the test question>} \\
%             % {\fontfamily{ppl}\selectfont \textbf{\#Hallucinated Answer\#:}} \\
%            \\ 
%             \bottomrule
% 	\end{tabular}
% 	\caption{Representative examples for these prompts of different categories.} 
%         % \vspace{-0.2cm}
% 	\label{tab:prompt}
% \end{table*}

\begin{figure*}
\centering
\includegraphics[width=1\textwidth]{figure/felm_examples.png}
\caption{
    Representative examples of different domains in FELM.
} 
\label{fig:domain}
\end{figure*}
